Fate of a remnant solid disk around an eccentric giant planet

The composition of giant planets' atmospheres is an important tracer of their formation history. While many theoretical studies investigate the heavy-element accretion within a gaseous protoplanetary disk, the possibility of solid accretion after disk dissipation has not been explored. Here, we focus on the case of a gas giant planet excited to an eccentric orbit and assess the likelihood of solid accretion after disk dissipation. We perform N-body simulations of planetesimals and embryos around an eccentric giant planet. We consider various sizes and orbits for the eccentric planet and determine the fate of planetesimals and embryos. We find that the orbital evolution of solids, such as planetesimals and embryos, is regulated by weak encounters with the eccentric planet rather than strong close encounters. Even in the region where the Safronov number is smaller than unity, most solid materials fall onto the central star or are ejected from the planetary system. We also develop an analytical model of the solid accretion along the orbital evolution of a giant planet, where the accretion probability is obtained as a function of the planetary mass, radius, semi-major axis, eccentricity, inclination, and solid disk thickness. Our model predicts that $\sim$0.01-0.1 $M_\oplus$ of solids is accreted onto an eccentric planet orbiting in the outer disk ($\sim10$ au). The accreted heavy-element mass increases (decreases) with the eccentricity (inclination) of the planet. We also discuss the possibility of collisions of terrestrial planets and find that $\sim10\%$ of the hot Jupiters formed via high-eccentric migration collide with a planet of $10M_\oplus$. However, we find that solid accretion and collisions with terrestrial planets are minor events for planets in the inner orbit, and a different accretion process is required to enrich eccentric giant planets with heavy elements.

==> texts_old/evolvingPlanet.tex <==
In the previous section, we inferred the accretion probability of a giant planet with a fixed orbit without considering the planet's orbital evolution. 
Here, we investigate how the planet's eccentricity evolution affects the inferred accretion probability. 

\subsection{Eccentricity excitation}\label{sec:method_EccExcite}
\textcolor{blue}{
We consider a case where multiple planets orbit the exterior of the planetesimal disk.
The planets initiate orbital instability and increase eccentricities, and then the pericenter of the innermost planet starts to cross the planetesimals' orbit.
We assume that the gravitational interaction with the innermost planet is the dominant perturber onto the planetesimal disk and neglects the gravity from the outer planets since the gravitational force from the outer planets is much smaller than that from the innermost planet. %, which has the smallest pericenter $q_\mathrm{p}$,
}

We start the N-body simulations with $e_\mathrm{p}=0$ and increase the planetary eccentricity by $1/\tau_\mathrm{ecc}$ every orbit where $\tau_\mathrm{ecc}$ is the excitation timescale.
There are various mechanisms for eccentricity excitation, and the excitation timescale differs in each mechanism. 
Typical timescales of the Kozai-Lidov resonance and secular interactions could be $10^5 P_\mathrm{orb,p}$ or longer \citep[e.g.][]{Dawson+2018}.
On the other hand, planet-planet scattering can increase the eccentricity more quickly.
The eccentricity excitation kicked by a single encounter is given by: 
\begin{eqnarray}
    \Delta e &\lesssim& \frac{v_\mathrm{esc}}{v_\mathrm{K}}, \\
            &=& 0.32 \left( \frac{M_\mathrm{p}}{0.5M_\mathrm{Jup}} \right)^{1/2} \left( \frac{R_\mathrm{p}}{2 R_\mathrm{Jup}} \right)^{-1/2} \left( \frac{a_\mathrm{p}}{0.1 \mathrm{au}} \right)^{1/2} \left( \frac{M_\mathrm{s}}{M_\oplus} \right)^{-1/2}.
\end{eqnarray}
N-body simulations have shown that planet-planet scattering can excite the planetary eccentricity as quickly as $10^3 P_\mathrm{orb,p}$ at most \citep{Carrera+2019, Pu+2021, Garzon+2022}.
We consider the following values of  $\tau_\mathrm{ecc}=10^3, 10^4, 10^5 P_\mathrm{orb,p}$ to account for the various excitation mechanisms. 

While the secular interactions keep the semi-major axis constant \citep{Teyssandier+2019}, the planet-planet scattering changes other orbital parameters, such as the planetary semi-major axis and inclination \citep{Carrera+2019, Pu+2021, Garzon+2022}. 
However, here, we increase the eccentricity by keeping the semi-major axis and the inclination constant to investigate how the time evolution of the planetary pericenter affects the accretion probability.


\subsection{Orbital evolution of planetesimals before orbital crossing}\label{sec: OrbitalEvolutionBOC}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/EccExcite/result_psdEccp_rev.png}
    \caption{
    Same as fig.~\ref{fig: fitting} but with a planet whose eccentricity increases with a given timescale $\tau_\mathrm{ecc}$.
    The blue solid lines show the numerical results, and the green dashed lines show eq.~(\ref{eq: accretion_probability}).
    }
    \label{fig:collision_psdEccp}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:collision_psdEccp} shows the accretion fraction of planetesimals $F_\mathrm{acc}$ vs.~the initial semi-major axis of planetesimals.
When the eccentricity excitation is $\tau_\mathrm{ecc}=10^3 P_\mathrm{orb,p}$, $F_\mathrm{acc}$ exceeds $10\%$ in the inner disk $a<1 \mathrm{au}$ and around the initial orbit of the planet $a\sim10\mathrm{au}$.
When the planet's eccentricity is small, the gravitational focusing works effectively, and $F_\mathrm{acc}$ can be high. 
The planet crosses the orbits of planetesimals between the pericenter $a_\mathrm{p}(1-e_\mathrm{p})$ and apocenter $a_\mathrm{p}(1+e_\mathrm{p})$.
When the planetary eccentricity is small, the sweeping area is also small. 
As the planet is excited to the eccentric orbit, the planet can accrete planetesimals in a wider orbit, but the accretion probability decreases because of the lower $F_\mathrm{grav}$.
This effect leads to a peak on $F_\mathrm{acc}$ around $a\sim a_\mathrm{p}$.
On the other hand, $F_\mathrm{acc}$ is higher in the inner disk, too, because $R_\mathrm{p}/b_\mathrm{close}$ is larger there.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \begin{center}
    \includegraphics[width=150mm]{fig/EccExcite/Snapshots_TauEcc_rev.png}
    \caption{
    Snapshots of the planetesimal disk when the planet's eccentricity increases with time.
    The left and right columns show the cases with $\tau_\mathrm{ecc}=10^3 P_\mathrm{orb,p}$ and $10^3 P_\mathrm{orb,p}$, respectively.
    The upper and lower panels show the snapshots when the planetary eccentricity is $e_\mathrm{p}=0.3$ and $0.81$, respectively.
    The vertical dotted lines are the pericenter and apocenter of the planet.
    The dashed lines are the analytical models of the planetesimal eccentricity given by eq.~(\ref{eq:ecc_PassingStarEvolv}).
    When $\tau_\mathrm{ecc}=10^5 P_\mathrm{orb,p}$, the planetesimal eccentricity is smaller than that given by eq.~(\ref{eq:ecc_PassingStarEvolv}) because the resonances suppress the linear increase of the eccentricity.
    }
    \label{fig: Snapshots_psdEccp}
  \end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

When the eccentricity excitation is slow as $\tau_\mathrm{ecc}=10^4 P_\mathrm{orb,p}$ and $10^5 P_\mathrm{orb,p}$, the accretion fraction in the inner orbit is reduced and opens a gap.
This is because some planetesimals are eliminated from the planetary system before the planet crosses the orbits of planetesimals.
\cite{Kobayashi+2001} showed that the eccentric object can perturb the inner planetesimal disk without orbital crossing.
The eccentricity perturbation put by a passing object is given as \citep{Kobayashi+2001}:
\begin{eqnarray}
    \Delta e_\mathrm{pass} &\simeq& A \left( \frac{a}{q_\mathrm{p}} \right)^{5/2},  \label{eq:ecc_PassingStar} \\
    A &=& \frac{15 \pi}{32 \sqrt{2}}  \frac{M_\mathrm{p}/M_\mathrm{s}}{\sqrt{1+M_\mathrm{p}/M_\mathrm{s}}} 
    \left[ \cos^2 \omega_\mathrm{p} \left(1-\frac{5}{4} \sin^2 i_\mathrm{p}\right)^2 \right. \nonumber \\
    && \left. + \sin^2\omega_\mathrm{p} \cos^2 i_\mathrm{p} \left(1-\frac{15}{4} \sin^2 i_\mathrm{p}\right)^2 \right]^{1/2}, \label{eq:ecc_PassingStar2}
\end{eqnarray} 
where $q_\mathrm{p}$ is the pericenter of the planet.
We adopt eq.~(\ref{eq:ecc_PassingStar}) to the eccentric planet and integrate it along the planetary eccentricity evolution.  
We obtain the eccentricity of the planetesimal disk, which is given by: 
\begin{eqnarray}
    \left \langle e \right \rangle &\simeq& \int_0^{t} \Delta e_\mathrm{pass} \mathrm{d} t^\prime = \int_0^{e_\mathrm{p}} \Delta e_\mathrm{pass} \frac{\tau_\mathrm{ecc}}{P_\mathrm{orb,p}} \mathrm{d} e_\mathrm{p}^\prime, \nonumber \\
    &=& \left \langle e_0 \right \rangle +\frac{2}{3} A \tau_\mathrm{ecc} \left(\frac{a}{a_\mathrm{p}}\right)^{5/2} \left[ \left( 1- e_\mathrm{p} \right)^{-3/2} -1 \right]. \label{eq:ecc_PassingStarEvolv}
\end{eqnarray}
Left panels of Fig.~\ref{fig: Snapshots_psdEccp} show snapshots of the planetesimal disk when $\tau_\mathrm{ecc}=10^3 P_\mathrm{orb,p}$.
We find that eq.~(\ref{eq:ecc_PassingStarEvolv}) reproduces well the eccentricity evolution of the planetesimals.
%when $\tau_\mathrm{ecc}=10^3 P_\mathrm{orb,p}$.
The condition where the planet crosses the orbit of planetesimals is given by: 
\begin{eqnarray}    
    a \left(1+e\right) = a_\mathrm{p} \left( 1-e_\mathrm{p} \right). \label{eq:orbits_crossed}
\end{eqnarray}
By solving eq.~(\ref{eq:ecc_PassingStarEvolv}) and eq.~(\ref{eq:orbits_crossed}) numerically, we can obtain the eccentricity of planetesimals and the planet when the orbits are crossed $e_\mathrm{cross}$, and $e_\mathrm{cross,p}$, separately.
As $e_\mathrm{cross}$ increases, the mean ejection time given by eq.~(\ref{eq:stay_time}) decreases, which leads to a decrease in the accretion probability. 
If $e_\mathrm{cross}$ is close to $1$, planetesimals are eliminated from the planetary system without crossing their orbits with that of the planet, and the accretion probability drops to zero.
When $\tau_\mathrm{ecc}=10^3 P_\mathrm{orb,p}$, $e_\mathrm{cross}$ is $\lesssim0.1$, and almost all planetesimals can stay in the planetary system until their orbits cross to that of a planet.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/EccExcite/Ecross.png}
    \caption{
    $r_\mathrm{cross}=a_\mathrm{p}(1-e_\mathrm{cross,p})$ vs. $e_\mathrm{cross}$ obtained by the N-body simulations.
    $e_\mathrm{cross}$ and $e_\mathrm{cross,p}$ are calculated by taking the average of eccentricities of planetesimals whose orbits are just before crossing to the planet's orbit.
    The dashed lines show $e_\mathrm{cross}$ obtained from eq.~(\ref{eq:ecc_PassingStarEvolv}) and eq.~(\ref{eq:orbits_crossed}).
    The thick dashed lines represent eq.~(\ref{eq:acrit}). 
    When eq.~(\ref{eq:acrit}) is not achieved, the analytical expression reproduces the numerical results well.
    The different colors correspond to the different eccentricity excitation timescales $\tau_\mathrm{ecc}$ as indicated in the legend.}
    \label{fig: Ecross}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Right panels of Fig.~\ref{fig: Snapshots_psdEccp} show snapshots when $\tau_\mathrm{ecc}=10^5 P_\mathrm{orb,p}$.
The eccentricity is smaller than that estimated by eq.~(\ref{eq:ecc_PassingStarEvolv}) where $a\gtrsim1.4 \au$ for $e_\mathrm{p}=0.3$ and $a\gtrsim0.39 \au$ for $e_\mathrm{p}=0.8$.
This is because of the effect of secular resonances.
\citet{Kobayashi+2001} found that resonance effects appear around $r/q_\mathrm{p}\gtrsim0.2$.
This resonance effects suppress the eccentricity excitation.
%While the eccentricity perturbation accumulates linearly, resonance effects suppress the eccentricity excitation.
%\citet{Kobayashi+2001} found that resonance effects appear around $r/q_\mathrm{p}\gtrsim0.2$.
%The right panels of Fig.~\ref{fig: Snapshots_psdEccp} show snapshots when $\tau_\mathrm{ecc}=10^5 P_\mathrm{orb,p}$, and the resonances appear $a\gtrsim1.4 \au$ for $e_\mathrm{p}=0.3$ and $a\gtrsim0.39 \au$ for $e_\mathrm{p}=0.8$.
%Due to the resonance effect, the eccentricity is smaller than that estimated by eq.~(\ref{eq:ecc_PassingStarEvolv}).
By analyzing the eccentricity evolution of each planetesimal, we find that the typical timescale of the resonance $\tau_\mathrm{res, sup}$ is $\sim10^3~\mathrm{years}$ (see details in Appendix~\ref{app: resonances}). 
If the timescale of the resonance crossing the disk $\tau_\mathrm{res, cross} = a/\dot{q}_\mathrm{p}$ is longer than $\tau_\mathrm{res, sup}$, the resonances can effectively suppress the eccentricity excitation of the planetesimal disk and reduce $e_\mathrm{cross}$.
The resonances become effective when %a>a_\mathrm{cirt}$ and $a_\mathrm{cirt}$ is given by: 
\begin{eqnarray}
    a_0 > a_\mathrm{cirt} = \frac{\tau_\mathrm{res, sup}}{\tau_\mathrm{ecc}} a_\mathrm{p}. \label{eq:acrit}
\end{eqnarray}
 
Figure~\ref{fig: Ecross} shows $r_\mathrm{cross}=a_\mathrm{p}(1-e_\mathrm{cross,p})$ and $e_\mathrm{cross}$ as inferred from  the N-body simulations.
$e_\mathrm{cross}$ and $e_\mathrm{cross,p}$ are obtained by calculating the mean eccentricity of planetesimals whose orbits are just before crossing to the planet's orbit: $0.8<a(1+e)/a_\mathrm{p}(1-e_\mathrm{p})<0.9$.
The dashed lines show $e_\mathrm{cross}$ obtained from  eq.~(\ref{eq:ecc_PassingStarEvolv}) and eq.~(\ref{eq:orbits_crossed}). 
The thick dashed lines correspond to the cases when $a_0>a_\mathrm{cirt}$. %eq.~(\ref{eq:acrit})$
%Substituting $\tau_\mathrm{res, sup}=10^3 P_\mathrm{orb}$, we get $a_\mathrm{cirt}=1 \au$ for $\tau_\mathrm{ecc}=10^4 P_\mathrm{orb,p}$ and $a_\mathrm{cirt}=0.1\au$ for $\tau_\mathrm{ecc}=10^5 P_\mathrm{orb,p}$, which are consistent with the centers of the gaps found in $F_\mathrm{acc}$.
When $a_0<a_\mathrm{cirt}$, $e_\mathrm{cross}$ increases with increasing $r_\mathrm{cross}$
and eq.~(\ref{eq:ecc_PassingStarEvolv}) and eq.~(\ref{eq:orbits_crossed}) reproduce $e_\mathrm{cross}$ well. 
On the other hand, when $a_0>a_\mathrm{cirt}$, $e_\mathrm{cross}$ decreases with increasing $r_\mathrm{cross}$ because the resonances become effective.
We find that the gaps in $F_\mathrm{acc}$ open when $e_\mathrm{cross}\sim 0.3$.
%and $a_0<a_\mathrm{cirt}$.
%{\bf please check... }
%Therefore, $e_\mathrm{cross}$ has a peak around $a_0 \sim a_\mathrm{cirt}$.


\subsection{Accretion probability by an eccentric planet}
%When we include this gap-opening effect 
Finally, we model the accretion probability of planetesimals with the initial semi-major axis $a_\mathrm{0}$ by %and the semi-major axis of planet $a_\mathrm{p}$ , a_\mathrm{p}
\begin{eqnarray}\label{eq: accretion_probability}
    P_\mathrm{acc} (a_\mathrm{0})=
    \begin{cases}
          P_\mathrm{acc}^\prime (r=r_\mathrm{cross},e_\mathrm{p}=e_\mathrm{p,cross}) \\
        ~\text{~for~} \tau_\mathrm{res, cross} < \tau_\mathrm{res, sup} \text{~and~} e_\mathrm{cross} < e_\mathrm{cross,crit}, \\
         0 
        \text{~other~},
    \end{cases}
\end{eqnarray}
%with
%\begin{eqnarray}
%    r_\mathrm{cross} &=& a_\mathrm{0} (1+e_\mathrm{cross}),
    %e_\mathrm{p} &=& e_\mathrm{cross,p},
%\end{eqnarray}
where we set $\tau_\mathrm{res, sup}=2\times10^3 P_\mathrm{orb}$ and $e_\mathrm{cross,crit}=0.3$ from the numerical results. 
$r_\mathrm{cross}$, $e_\mathrm{cross}$ and $e_\mathrm{p,cross}$ are obtained with eq. (44) and eq. (45) by substituting $a=a_\mathrm{0}$.
Other parameters such as $M_\mathrm{p}$, $R_\mathrm{p}$, $a_\mathrm{p}$, $\sin i_\mathrm{p}$ and $\left \langle \sin^2 i_\mathrm{0} \right \rangle^{1/2}$ are input parameters. %disk parameters such as
Our model can reproduce the obtained accretion fraction (see Fig.~\ref{fig:collision_psdEccp}).




==> texts_old/fixedPlanet.tex <==
In order to assess the accretion probability, we investigate the orbital evolution of planetesimals and embryos around an eccentric planet. 
Using N-body simulations, we derive a formula for the accretion probability for a giant planet with a fixed orbit. 

\subsection{Numerical Setup}
We integrate orbits of planetesimals and embryos around a central star with a mass of $M_\mathrm{s}$ and with an eccentric protoplanet with a mass of $M_\mathrm{p}$. 
The semi-major axis $a_\mathrm{p}$ and the eccentricity $e_\mathrm{p}$ of the planet are set as input parameters.
%perihelion of the eccentric planet at $q_\mathrm{p}$.
%The semi-major axis of the eccentric protoplanet $a_\mathrm{p}$ is set as an input parameter.
In this case, the perihelion and apohelion of the planet are $a_\mathrm{p} (1-e_\mathrm{p})$ and $a_\mathrm{p} (1+e_\mathrm{p})$.
The inclination $\sin i_\mathrm{p}$ is also an input parameter.
The other orbital angles, longitude of ascending node $\Omega_\mathrm{p}$, longitude of pericentre $\varpi_\mathrm{p}$, and true anomaly $\tau_\mathrm{p}$, are set as $(\Omega_\mathrm{p},\varpi_\mathrm{p},\tau_\mathrm{p})=(0,0,\pi)$ or $(0,1/2\pi,\pi)$.
We distribute planetesimals and embryos around the eccentric planet and integrate the orbits up to a time  $t=10^6 \yr$, or until all the particles other than the planet have been eliminated from the simulations.
In our simulations, we use the IAS 15 integrator \citep{Everhart+1985, Rein+2015}, whose accuracy is sufficiently high to calculate the orbital evolution of eccentric objects. 
The benchmark results of our simulations are described in appendix \ref{app: Integrator}. 

We count the number of particles that collide with the eccentric protoplanet $N_\mathrm{col}$, fall to the central star $N_\mathrm{fall}$, and are ejected from the planetary system $N_\mathrm{eject}$.
We judge that a particle collides with the eccentric protoplanet once the relative distance becomes smaller than the physical radius of the planet $R_\mathrm{p}$.
A particle whose orbital distance from the central star $r$ becomes smaller than the central star's radius $R_\mathrm{star} = 0.0046 \au$ (comparable to the solar radius) is assumed to fall into the central star. 
Once $r>10^3 \au$ is achieved, the particle is assumed to be eliminated from the planetary system.


\subsection{Planetesimal accretion by a giant planet from a planetesimal  disk}\label{sec: CollisionProbability}

First, we consider that a planetesimal disk has remained after disk dissipation. 
We assume that the planetesimals are distributed uniformly in logarithmic space in the radial direction. 
We distribute planetesimals from $a_\mathrm{pl,in}$ to $a_\mathrm{pl,out}$, where $a_\mathrm{pl,in}$ is set as smaller than $a_\mathrm{p}(1-e_\mathrm{p})$, and $a_\mathrm{pl,out}$ is set as larger than $a_\mathrm{p}(1+e_\mathrm{p})$.
The eccentricity and inclination are then given by Rayleigh distribution with the eccentricity dispersion $\langle e_0^2 \rangle^{1/2}$ and inclination dispersion $\langle \sin ^2 i_0 \rangle^{1/2}$.
The other orbital angles of planetesimals, the longitude of ascending node $\Omega$, the longitude of pericentre $\varpi$, and true anomaly $\tau$, are chosen randomly.

To reduce the computational cost, the planetesimals are treated as test particles. 
Since planetesimals are represented by test particles, our results can also be applied to solid disks of smaller particles like debris and dust. 
The number of test particles $N_\mathrm{tp}$ is set so that more than 400 particles are in each bin with a width of 0.1 in logarithmic space in the radial direction. 
At the end of simulations, some planetesimals remain in the system.
However, we stop the simulations at $t=10^6 \yr$ because planetesimal accretions with the protoplanet mainly occur around $t\lesssim10^5~\yr$. % (see \ref{app:Integrator}).
Therefore, our numerical results are unexpected to change if longer simulation times are considered. 

\begin{table*}%[h]
	\centering
	\begin{tabular}{ c|c|c|c } % four columns, alignment for each p{5 cm}
		\hline
		& parameter & standard value & parameter study \\
		\hline
        $M_\mathrm{s}$   & mass of central star & $M_\odot$ & \\
    	$M_\mathrm{p}$   & mass of protoplanet & $M_\mathrm{Jup}$ & $1/8 M_\mathrm{Jup}$-$8 M_\mathrm{Jup}$  \\
    	$R_\mathrm{p}$   & radius of protoplanet & $R_\mathrm{Jup}$ & $1/8 R_\mathrm{Jup}$-$R_\mathrm{Jup}$ \\
    	$a_\mathrm{p}$   & semi-major axis of protoplanet & $1 \au$ & $1 \au$, $10 \au$ \\
    	$e_\mathrm{p}$   & eccentricity of protoplanet & $0.99$ & $0.1$-$0.99$ \\
    	$\sin i_\mathrm{p}$   & inclination of protoplanet & $0$ & $0,10^{-3},10^{-2}$ \\
    	$\varpi_\mathrm{p}$ & longitude of pericenter of protoplanet & $0$ & $0,1/2\pi$ \\
    		\hline
		$a_\mathrm{pl,in}$ & inner edge of planetesimal disk & $0.01 \au$ & $0.01$-$0.1$ \\
		$a_\mathrm{pl,out}$ & outer edge of planetesimal disk & $3 \au$ & $3$-$25 \au$ \\
        $\langle e_0^2 \rangle^{1/2}$ & initial eccentricity dispersion of planetesimals & $10^{-3}$ & \\
        $\langle \sin^2 i_0 \rangle^{1/2}$ & initial inclination dispersion of planetesimals & $0.5\times10^{-3}$ & $10^{-4}$-$10^{-1}$ \\
		\hline
	\end{tabular}
	\caption{
	The various parameters used in this study (see text for details). 
    }
    \label{tb:parameters}
%}
\end{table*}

We perform parameter studies where we change  $M_\mathrm{p}$, $R_\mathrm{p}$, $a_\mathrm{p}$, and  $e_\mathrm{p}$, which are also parameterised in \citet{Rodet+2023}.
We also perform parameter studies where we vary  $\sin i_\mathrm{p}$, and $\langle \sin^2 i_0 \rangle^{1/2}$. 
The values of the different parameters used in our simulations as well as the range of parameters are listed in Table ~\ref{tb:parameters}. 


\subsubsection{Orbital evolution around an eccentric giant planet}\label{sec:standard}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \begin{center}
    \includegraphics[width=180mm]{fig/EccPlanet/snapshots.png}
    \caption{
    Snapshots of orbital integration around an eccentric giant planet.
    The left and right columns show the eccentricity and inclination, respectively, with the semi-major axis of planetesimals.
    Time progresses from upper to lower panels.
    The solid lines in the left column show $e_\mathrm{fall}$.
    The small boxes on the right side of each panel show the histogram.
    The total number of planetesimals $N$ is written in the boxes.
    Here, we show the case with $a_\mathrm{p}=1 \au$, $e_\mathrm{p}=0.99$, $\sin i_\mathrm{p}=0$, $M_\mathrm{p}=M_\mathrm{Jup}$ and $R_\mathrm{p}=R_\mathrm{Jup}$.
    }
    \label{fig:snapshots}
  \end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%{\bf FIX: We begin with an extreme case of $e_\mathrm{p}=0.99$ since the extreme case has lots of important information about orbital evolution. }
Figure~\ref{fig:snapshots} shows the snapshots from our simulation.
We present the case with a planet of $M_\mathrm{p}=M_\mathrm{Jup}$, $R_\mathrm{p}=R_\mathrm{Jup}$, and an orbit with $a_\mathrm{p}=1 \au$, $e_\mathrm{p}=0.99$, $\sin i_\mathrm{p}=0$.
The eccentricity of the entire planetesimal disk is excited by the first passage of the eccentric planet.
Eccentricity excitation occurs every orbit and uniformly within the planetesimal disk.
In a-particle-in-a-box approximation, a velocity perturbation by the passing planet is given by \citep[e.g.][]{Armitage2010}: 
\begin{eqnarray}
    \delta v \sim \frac{2 \mathcal{G} M_\mathrm{p}}{b v_\mathrm{rel}}, \label{eq:deltav}
\end{eqnarray}    
where $\mathcal{G}$ is the gravitational constant, $b$ is the impact parameter, and $v_\mathrm{rel}$ is the relative velocity to the passing planet.
Here, we assume that the impact parameter is the order of the orbital radius of the perturbed planetesimal $a$, and the relative velocity is $e_\mathrm{p} v_\mathrm{K} (a)$ which are reasonable approximations. 
The weak perturbation from the passing planet is given by: 
\begin{eqnarray}
    \delta v_\mathrm{weak} \sim v_\mathrm{K} (a) \frac{2}{e_\mathrm{p}}  \frac{M_\mathrm{p}}{M_\mathrm{s}}, \label{eq:deltav_far}
\end{eqnarray}
and the eccentricity perturbation on a planetesimal is approximated to be:  
\begin{eqnarray}
    \delta e_\mathrm{weak} \sim C_\mathrm{v} \frac{\delta v_\mathrm{weak}}{v_\mathrm{K} (a)} = \frac{2 C_\mathrm{v}}{e_\mathrm{p}} \frac{M_\mathrm{p}}{M_\mathrm{s}}, \label{eq:decc_weak}
\end{eqnarray}
where $C_\mathrm{v}$ is a fitting parameter.
The eccentricity excitation occurs in every orbit of the eccentric planet, and the excitation rate is independent of the radial distance from the central star.
Due to the large mass difference between the planet and planetesimals, the perturbations increase the eccentricity of the planetesimals linearly.
The eccentricity evolution can be written as: 
\begin{eqnarray}
    \frac{\mathrm{d} \left \langle e \right \rangle}{\mathrm{d} t} &\sim& \frac{\Delta e}{\Delta t} = \frac{\delta e_\mathrm{weak}}{P_\mathrm{orb,p}}, \\
    \left \langle e \right \rangle &\sim& \left \langle {e_0}^2 \right \rangle^{1/2} + \delta e_\mathrm{weak} \frac{t}{P_\mathrm{orb,p}}, \label{eq:TimeEvolution_Ecc}
\end{eqnarray}
where $P_\mathrm{orb,p}$ is the orbital period of the eccentric planet.


On the other hand, the inclination of planetesimals is barely changed at $t\lesssim10 P_\mathrm{orb,p}$. 
Inclination excitation requires close encounters with the eccentric planet.
When the eccentric planet passes through the planetesimal disk $\sin i_\mathrm{p}<\sin i$, a z-component of the velocity perturbation is given by: 
\begin{eqnarray}
    \delta v_\perp = \delta v \frac{r \sin i}{b}.
\end{eqnarray}
We define the distance of the close encounter $b_\mathrm{close}$ as the distance at which the velocity perturbation doubles the planetesimal's inclination.
Therefore, 
\begin{eqnarray}
    C_\mathrm{v} \frac{\delta v_\perp}{v_\mathrm{K}} &=& \sin i, \\
    \frac{b_\mathrm{close}}{r} &=& \sqrt{\frac{2 C_\mathrm{v}}{e_\mathrm{p}} \frac{M_\mathrm{p}}{M_\mathrm{s}}}, \\
                     &=& 0.062 \left(\frac{C_\mathrm{v}}{2}\right)^{1/2} \left(\frac{e_\mathrm{p}}{0.99} \right)^{-1/2} \left( \frac{M_\mathrm{p}}{M_\mathrm{Jup}} \right)^{1/2} \left( \frac{M_\mathrm{s}}{M_\odot} \right)^{-1/2}.
\end{eqnarray}
At the beginning of the simulation, the thickness of the planetesimal disk $r \sin i$ is smaller than $b_\mathrm{close}$.
The typical timescale of the close encounter $\tau_\mathrm{close,2D}$ is given by: 
\begin{eqnarray}
    \tau_\mathrm{close,2D} &=& \frac{2 \pi r}{2 b_\mathrm{close}} P_\mathrm{orb,p}, \\
    &\sim& 51 P_\mathrm{orb,p} \left(\frac{C_\mathrm{v}}{2}\right)^{-1/2} \left(\frac{e_\mathrm{p}}{0.99} \right)^{1/2} \left( \frac{M_\mathrm{p}}{M_\mathrm{Jup}} \right)^{-1/2} \left( \frac{M_\mathrm{s}}{M_\odot} \right)^{1/2}. \label{eq:tau_close_2D}
\end{eqnarray}
Equation~(\ref{eq:tau_close_2D}) is consistent with Fig.~\ref{fig:snapshots}, in which the inclination starts to increase around $t\sim10^2 P_\mathrm{orb,p}$.
Once the disk thickness exceeds $b_\mathrm{close}$, close encounters occur in three dimensions.  
In this case, the typical timescale of the close encounter $\tau_\mathrm{close,3D}$ is given by: 
\begin{eqnarray}
    \tau_\mathrm{close,3D} = \frac{2 \pi r \cdot r \sin i}{\pi {b_\mathrm{close}}^2 } P_\mathrm{orb,p}. \label{eq:tau_close_3D}
\end{eqnarray}
The time evolution of inclination can be written as: 
\begin{eqnarray}
    \frac{ \mathrm{d} \left \langle \sin i \right \rangle}{\mathrm{d} t} \sim \frac{\Delta \sin i}{\Delta t} = 
    \left\{  \begin{array}{ll}
        \frac{\left \langle \sin i \right \rangle}{\tau_\mathrm{close,2D}} & \mathrm{ for}~ \left \langle \sin i \right \rangle < \sin i_\mathrm{b} \\
        \frac{\left \langle \sin i \right \rangle}{\tau_\mathrm{close,3D}} & \mathrm{ for}~ \sin i_\mathrm{b} < \left \langle \sin i \right \rangle 
    \end{array} \right. , \\
    \left \langle \sin i \right \rangle \sim
        \left\{  \begin{array}{ll}
            \left \langle \sin i_0 \right \rangle \exp \left( \frac{t}{\tau_\mathrm{close,2D}} \right) & \mathrm{ for}~ \left \langle \sin i \right \rangle < \sin i_\mathrm{b} \\
            \frac{ {b_\mathrm{close}}^2}{4 r^2} \frac{t-t_\mathrm{b}}{P_\mathrm{orb,p}} + \sin i_\mathrm{b} & \mathrm{ for}~ \sin i_\mathrm{b} < \left \langle \sin i \right \rangle 
            \end{array} \right. ,
    \label{eq:TimeEvolution_Inc}
\end{eqnarray}    
with
\begin{eqnarray}
    \sin i_\mathrm{b} &=& \frac{b_\mathrm{close}}{r}, \\
    t_\mathrm{b} &=& \tau_\mathrm{close, 2D} \log \frac{\sin i_\mathrm{b}}{\left \langle \sin i_0 \right \rangle}.
\end{eqnarray}
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/EccPlanet/time_orbits_a10.png}
    \caption{
    Time evolution of the mean eccentricity (cross points) and inclination (square points) of planetesimals.
    The different colors correspond to different assumed masses for the eccentric planet.
    We also plot eq.~(\ref{eq:TimeEvolution_Ecc}) with solid lines and eq.~(\ref{eq:TimeEvolution_Inc}) with dashed lines using $C_v=2$.
    Here, we show the results obtained in the standard cases with $a_\mathrm{p}=10 \au$.
    }
    \label{fig:time_orbit}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Figure~\ref{fig:time_orbit} shows the time evolution of the 
geometric 
mean eccentricity and inclination of planetesimals for various assumed planetary masses.
We also plot eq.~(\ref{eq:TimeEvolution_Ecc}) and eq.~(\ref{eq:TimeEvolution_Inc}) with $C_v=2$.
We find that eq.~(\ref{eq:TimeEvolution_Ecc}) and eq.~(\ref{eq:TimeEvolution_Inc}) reproduce the numerical results well.


\subsubsection{Fate of planetesimals}\label{sec:fate_planetesimals}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/EccPlanet/result_Standard.png}
    \caption{
    The fate of planetesimals around the eccentric planet of $e_\mathrm{p}=0.99$. %$ with Jupiter-mass and radius.
    The fractions of collided (blue), dropped (green), and scattered (orange) planetesimals are plotted as a function of the initial semi-major axis of test particles.
    We take the width of bins as 0.1 in logarithm space.
    Here, we show the results obtained in the standard cases with $a_\mathrm{p}=1 \au$ (dashed line) and $a_\mathrm{p}=10 \au$ (solid lines).
    The vertical dashed line shows the location of $\Theta=1$.
    }
    \label{fig:fate_standard}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:fate_standard} shows the final fate of planetesimals as a function of their initial semi-major axes.
The blue, green, and orange lines show the fraction of planetesimals that accrete on the eccentric planet $F_\mathrm{acc}$, fall to the central star $F_\mathrm{fall}$, and are ejected from the planetary system $F_\mathrm{eject}$, respectively. 
In the inner disk region, most planetesimals are accreted by the eccentric planet. 
We also find that while $F_\mathrm{acc}$ is decreasing with the increasing semi-major axis of planetesimals, $F_\mathrm{fall}$ is increasing with the increasing semi-major axis of planetesimals.
Beyond a radial distance of $a\sim 0.1 \au$, planetesimals mostly end up falling into the central star.
Due to the weak gravitational bound from the central star, $F_\mathrm{eject}$ increases in the outer disk region.
However, the ejection from the planetary system is rare, and $F_\mathrm{eject}$ does not exceed $0.2$.

The Safronov number $\Theta = v_\mathrm{esc}^2 / 2 v_\mathrm{K}^2$ is usually used as an indicator for describing the fate of planetary objects in an unstable system.
An encounter grazing the planetary surface puts a velocity kick of $\sim v_\mathrm{esc}$ to a planetesimal, which leads to $\delta e \sim \sqrt{2 \Theta}$. 
If the Safronov number is larger than one, the gravitational scattering by the planet is likely to lead to ejection. 
Therefore, it is predicted that accretion is dominant in the region of $\Theta<1$ while ejection or falling into the star is dominant with $\Theta>1$. %\citet{Seligman+2022}
The orbital distance where $\Theta=1$ is given by:
\begin{eqnarray}
    r_\mathrm{\Theta,1} = 0.49 \au \left( \frac{R_\mathrm{p}}{R_\mathrm{Jup}} \right) \left( \frac{M_\mathrm{p}}{M_\mathrm{Jup}} \right)^{-1} \left( \frac{M_\mathrm{s}}{M_\odot} \right).
\end{eqnarray} 
The vertical dotted line in Fig.~\ref{fig:fate_standard} shows the location of $r_\mathrm{\Theta,1}$.
Our numerical results show that the fate of planetesimals is different from the one expected from the Safronov number because while a single close encounter at $r<r_\mathrm{\Theta,1}$ is insufficient to eject planetesimals, a series of weak encounters with the highly eccentric planet accumulate perturbations on the planetesimal's orbit which eventually leads to ejection. 



\subsubsection{accretion to close encounter ratio}\label{sec:fcc}
If the eccentricity exceeds $e_\mathrm{fall}=1-R_\mathrm{star}/a$ before accretion to the eccentric planet, the planetesimal will be removed from the planetary system by the falling or ejection.
The timescale at which planetesimals can remain in the planetary system is an important factor for the accretion probability. 
%The eccentricity with which planetesimals fall to the central star $e_\mathrm{fall}$ is given as $1-R_\mathrm{star}/a$.
By equating the mean eccentricity given by eq.~(\ref{eq:TimeEvolution_Ecc}) to $e_\mathrm{fall}$, we can obtain the duration time of the planetesimals in the system before they are eliminated $\tau_\mathrm{eject}$ as follows: 
\begin{eqnarray}
    %\left \langle e \right \rangle &=& e_\mathrm{fall}, \\
    \frac{\tau_\mathrm{eject}}{P_\mathrm{orb,p}} &=& \frac{1}{2 C_\mathrm{v}} \frac{M_\mathrm{s}}{M_\mathrm{p}} \left( 1 - \frac{R_\mathrm{star}}{a} \right). \label{eq:stay_time}
\end{eqnarray}
Figure~\ref{fig:stay_time} shows the geometric mean of the ejection time  
inferred in the numerical simulations.
The dotted lines show eq.~(\ref{eq:stay_time}).
Around the aphelion of the eccentric planet, $\tau_\mathrm{stay}$ gets higher than eq.~(\ref{eq:stay_time}) because some planetesimals stay in mean motion resonances, which delay the eccentricity excitation of the planetesimals.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/EccPlanet/stay_time.png}
    \caption{
    Averaged time before planetesimals fall to the central star or are ejected from the planetary system.
    Different colors correspond to the different masses of the eccentric planet.
    Square and cross plots show the cases with $a_\mathrm{p}=1 \au$ and $a_\mathrm{p}=10 \au$, respectively.
    The dotted lines show the analytical equation eq.~(\ref{eq:stay_time}) with a fitting parameter $C_\mathrm{v}=2$.
    }
    \label{fig:stay_time}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The planetesimal accretion probability depends on the geometry of the planetesimal disk.
%capture radius $R_\mathrm{cap}$.
The capture radius of an eccentric planet is given by: 
\begin{eqnarray}
    R_\mathrm{cap} = R_\mathrm{p} F_\mathrm{grav}  
                   = R_\mathrm{cap} \left( 1 + \frac{ {v_\mathrm{esc}}^2 }{ 2 {v_\mathrm{rel}}^2 } \right)^{1/2},
\end{eqnarray}
where $F_\mathrm{grav}$ is the gravitational focusing factor, $v_\mathrm{esc}$ and $v_\mathrm{rel}$ are the escape velocity of the planet and the relative velocity between the planet and planetesimals.
When the half thickness of the planetesimal disk $r \sin i$ is smaller than the capture radius $R_\mathrm{cap}$, particle accretion occurs two-dimensionally (2D).
The accretion probability per orbit of the eccentric planet  is given by: 
\begin{eqnarray}
    f_\mathrm{acc,2D} = \frac{R_\mathrm{cap}}{\pi r} \label{eq:fcol_2D}.
\end{eqnarray}
Once the thickness of the particle disk exceeds  $R_\mathrm{cap}$ the particle collision occurs in a 3D manner. 
The accretion probability is then given by: 
\begin{eqnarray}
    f_\mathrm{acc,3D} =  \frac{{R_\mathrm{cap}}^2}{4 \pi r^2 \sin i} \label{eq:fcol_3D}.
\end{eqnarray}

The close encounters with the eccentric planet increase the planetesimals' inclination.
%, which we define as encounters within $b_\mathrm{close}$.
The close encounter probability per planetary orbit is given by: 
\begin{eqnarray}
    f_\mathrm{close,2D} = \frac{b_\mathrm{close}}{\pi r}. \label{eq:fclose_2D}
\end{eqnarray}
When the thickness of the planetesimal disk exceeds $b_\mathrm{close}$ the close encounter probability is:
\begin{eqnarray}
    f_\mathrm{close,3D} =  \frac{{b_\mathrm{close}}^2}{4 \pi r^2 \sin i}. \label{eq:fclose_3D}
\end{eqnarray}

Using Eqs~(\ref{eq:fcol_2D}), (\ref{eq:fcol_3D}), (\ref{eq:fclose_2D}), and (\ref{eq:fclose_3D}), we obtain the accretion to close encounter fraction per single close encounter $f_\mathrm{a/c}$ to be: 
\begin{eqnarray}\label{eq:collision_to_scattering}
    f_\mathrm{a/c} =
        \begin{cases}
            \frac{f_\mathrm{acc,2D}}{f_\mathrm{close,2D}} = \frac{R_\mathrm{cap}}{b_\mathrm{close}} &\text{~for~} \sin i < \frac{R_\mathrm{cap}}{r}, \\
            \frac{f_\mathrm{acc,3D}}{f_\mathrm{close,2D}} = \frac{R_\mathrm{cap}}{b_\mathrm{close}} \frac{R_\mathrm{cap}}{r \sin i} &\text{~for~} \frac{R_\mathrm{cap}}{r} < \sin i < \frac{b_\mathrm{close}}{r}, \\
            \frac{f_\mathrm{acc,3D}}{f_\mathrm{close,3D}} = \left( \frac{ R_\mathrm{cap} }{b_\mathrm{close}} \right)^2 &\text{~for~} \frac{b_\mathrm{close}}{r} < \sin i. \\       
        \end{cases}
\end{eqnarray}
$f_\mathrm{a/c}$ depends on $R_\mathrm{cap}/b_\mathrm{close}$, which decreases with increasing radial distance from the central star. 
For a Jupiter mass planet with Jupiter's radius, $R_\mathrm{cap}/b_\mathrm{close}$ is $\sim0.76$, $0.082$ and $0.013$ at $r=0.01 \au$, $0.1 \au$ and $1\au$, respectively.
The typical timescale of a close encounter $\tau_\mathrm{close,2D}$ is shorter than the mean ejection time $\tau_\mathrm{eject}$.
Therefore, planetesimals are expected to experience a close encounter before they are removed from the planetary system.
$R_\mathrm{cap}/b_\mathrm{close}$ is qualitatively comparable to $F_\mathrm{acc}$.


\subsubsection{Fitting the numerical results}
%\subsubsection{Dependence on planetary parameters}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \begin{center}
    \includegraphics[width=160mm]{fig/EccPlanet/results_Fit.png}
    \caption{
    The fraction of collided particles $F_\mathrm{acc}$ as a function of the initial semi-major axis of planetesimals.
    We plot the results of parameter studies for different assumed planetary radius $R_\mathrm{p}$, the planetary mass $M_\mathrm{p}$, the planetary eccentricity $e_\mathrm{p}$, and the initial disk thickness $\left \langle \sin^2 i_0 \right \rangle^{1/2}$ from top to bottom.
    The left and right columns show the cases with $a_\mathrm{p}=1\au$ and $a_\mathrm{p}=10\au$, respectively.
    The solid lines show the fitting formula given by eq.~(\ref{eq:Pcol}).
    }
    \label{fig:fitting}
  \end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Figure~\ref{fig:fitting} shows the dependence of the accretion fraction of planetesimals $F_\mathrm{acc}$ (as a function of radial distance) on the assumed planetary radius $R_\mathrm{p}$, mass $M_\mathrm{p}$, eccentricity $e_\mathrm{p}$, and the initial inclination of the planetesimal disk $\sin i_0$. 
The accretion probability increases with increasing $R_\mathrm{p}$ and decreases with increasing $M_\mathrm{p}$ and $e_\mathrm{p}$, which are consistent with the results by \citet{Rodet+2023}.
We also find that the accretion probability decreases when the initial semi-major axis of planetesimal $a_0$ and the initial inclination $\sin i_0$ increase because the geometrical picture of accretion changes from 2D to 3D. 

We find that the accretion probability of planetesimals $P_\mathrm{col}^\prime$ is given by:
\begin{eqnarray}\label{eq:Pcol}
    P^\prime_\mathrm{col} &= \min( 1, P^{\prime\prime}_\mathrm{col}),
\end{eqnarray}
with
\begin{eqnarray}
    P^{\prime\prime}_\mathrm{col} &=& \int_0^{\tau_\mathrm{eject}} \frac{f_{a/c}}{\tau_\mathrm{close}} \mathrm{d} t, \\
                          &=& \alpha P_\mathrm{2D} +\beta P_\mathrm{3D2D} +\gamma P_\mathrm{3D},
\end{eqnarray}
where $\alpha$, $\beta$ and $\gamma$ are fitting parameters, and
\begin{align}
    P_\mathrm{2D} =
    \begin{cases}
          \frac{R_\mathrm{cap}}{b_\mathrm{close}} \log \frac{R_\mathrm{cap}}{r \left \langle \sin i_0 \right \rangle}
        &\text{~for~} \left \langle \sin i_0 \right \rangle < \frac{R_\mathrm{cap}}{r}, \\
         0
        &\text{~other~}. \\
    \end{cases} %\\
\end{align}
    %
    %
    %
\begin{align}
    P_\mathrm{3D2D} =
    \begin{cases}
          \frac{R_\mathrm{cap}}{b_\mathrm{close}} \left(1-\frac{R_\mathrm{cap}}{b_\mathrm{close}} \right)
        &\text{~for~} \left \langle \sin i_0 \right \rangle < \frac{R_\mathrm{cap}}{r}, \\
          \frac{R_\mathrm{cap}}{b_\mathrm{close}} \left(\frac{R_\mathrm{cap}}{r \left \langle \sin i_0 \right \rangle}-\frac{R_\mathrm{cap}}{b_\mathrm{close}} \right)
        &\text{~for~} \frac{R_\mathrm{cap}}{r} < \left \langle \sin i_0 \right \rangle < \frac{b_\mathrm{close}}{r}, \\
         0
        &\text{~other~}. \\
    \end{cases} %\\
\end{align}
    %
    %
    %
\begin{align}
    P_\mathrm{3D} =
    \begin{cases}
          \left( \frac{R_\mathrm{cap}}{b_\mathrm{close}} \right)^2 
            &\log \left\{ \frac{1}{4} \frac{b_\mathrm{close}}{r} \left( \frac{\tau_\mathrm{eject}}{P_\mathrm{orb,p}}-\pi \log \frac{\sin i_\mathrm{b}}{\left \langle \sin i_0 \right \rangle} \right) + 1 \right\} \\
          &\text{~for~} \left \langle \sin i_0 \right \rangle < \frac{b_\mathrm{close}}{r}, \\
          \left( \frac{R_\mathrm{cap}}{b_\mathrm{close}} \right)^2 
            &\log \left\{ \frac{1}{4 \left \langle \sin i_0 \right \rangle} \left(\frac{b_\mathrm{close}}{r}\right)^2 \frac{\tau_\mathrm{eject}}{P_\mathrm{orb,p}} + 1 \right\} \\
          &\text{~other~}. \\
    \end{cases}
\end{align}
We fit the above equations to the numerical results in logarithmic space substituting $r=a_0$.
The inferred fitting parameters are listed in table~\ref{tb:fitting_parameters} with the coefficient of determination being $0.951$. %3153826427119$.

Equation~(\ref{eq:Pcol}) reproduces the numerical results except in the cases of low planetary eccentricity $e_\mathrm{p}\lesssim0.3$.
Our model underestimates the accretion probability of $e_\mathrm{p}\lesssim0.3$.
This is because the orbital evolution of planetesimals becomes slower than eqs.~(\ref{eq:TimeEvolution_Ecc}) and (\ref{eq:TimeEvolution_Inc}) when $e_\mathrm{p} > \left \langle e \right \rangle$.
We discuss this point further in Sec.~\ref{sec: discussion_model}. 

\begin{table}%[h]
	\centering
	\begin{tabular}{ c|c } % four columns, alignment for each p{5 cm}
		\hline
		parameter & obtained value \\
		\hline
        $\alpha$   &  0.358 \\ %67944097999055 \\
        $\beta$   &  4.73 \\ %1433531451034 \\
        $\gamma$   &  7.81 \\ %2472463730468\\
		\hline
	\end{tabular}
	\caption{
	Fitting parameters obtained from the numerical simulations
    }
    \label{tb:fitting_parameters}
%}
\end{table}
%*Result************
%a0 =  0.35867944097999055 +- 0.07907931619129609
%a1 =  4.731433531451034 +- 0.11452183574178317
%a2 =  7.812472463730468 +- 0.7089450212170642
%*******************
%0.9513153826427119

\subsubsection{Dependence on the planetary inclination} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}
  \begin{center}
    \includegraphics[width=160mm]{fig/EccPlanet/result_psIncp.png}
    \caption{
    Same as Fig.~\ref{fig:fitting} but for different assumed planetary inclinations. 
    The blue and green solid lines show the cases with different longitudes of pericenter $\varpi_\mathrm{p}$.
    The orange dashed line shows the result for a non-inclined planet but with an inclination-excited planetesimal disk.}
    \label{fig:result_IncpIncpl}
  \end{center}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We considered the cases where the inclination of the eccentric planet is aligned to the planetesimal disk $\sin i_\mathrm{p}=0$.
If the eccentric planet is more inclined than the planetesimal disk $\sin i_\mathrm{p} > \left \langle \sin i \right \rangle$, the distance of the close encounter is: 
\begin{eqnarray}
    C_\mathrm{v} \frac{\delta v}{v_\mathrm{K}} \frac{r \sin i_\mathrm{p}}{{b_\mathrm{close}}^{\prime}} &=& \sin i, \\
    {b_\mathrm{close}}^{\prime} &=& {b_\mathrm{close}} \sqrt{\frac{\sin i_\mathrm{p}}{\sin i}}.
\end{eqnarray}
The inclination evolution accelerates by the factor of $\sqrt{\sin i_\mathrm{p}/\sin i}$.
However, the planetesimal disk reaches $\sin i_\mathrm{p}<\left \langle \sin i \right \rangle$ within $\tau_\mathrm{eject}$, and the following orbital evolution would be the same as the cases with $\sin i_\mathrm{p}<\left \langle \sin i \right \rangle$.
Figure~\ref{fig:result_IncpIncpl} shows the numerical results with $\sin i_\mathrm{p}=10^{-3}$ and $10^{-2}$.
For comparison, we also plot the results with $\sin i_\mathrm{p}=0$, but with $\left \langle \sin^2 i_0 \right \rangle^{1/2}=10^{-3}$ and $10^{-2}$. 
We find that the collision fraction with different $\sin i_\mathrm{p}$ is consistent with the cases of corresponding $\left \langle \sin^2 i_0 \right \rangle^{1/2}$ within a factor of $\sim2$.  
We also change the longitude of the pericenter $\varpi_\mathrm{p}$ and find that the collision fraction is mostly independent of  $\varpi_\mathrm{p}$. 
For the cases with $\sin i_\mathrm{p} > \left \langle \sin i_0 \right \rangle$ the collision probability is given by $P_\mathrm{col}^\prime$ with $\sin i_\mathrm{p}$ substituted for $\left \langle \sin i_0 \right \rangle$.

%\bf{Ravit stopped here}\\
\subsubsection{Effects of self-gravity}\label{sec:SelfGravity}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/Multi/time_orbits_ap10.png}
    \caption{
    Same as Fig.~\ref{fig:time_orbit}, but using embryos instead of a planetesimal disk.
    The blue and green plots show the geometrical mean of eccentricities and inclinations of embryos.
    The blue solid line shows eq.~(\ref{eq:TimeEvolution_Ecc}) with $\langle e_0 \rangle=1\times10^{-3}$.
    The green solid and dashed lines show eq.~(\ref{eq:TimeEvolution_Inc}) with $\langle \sin i_0 \rangle = 5 \times 10^{-4}$ and $\langle \sin i_0 \rangle = h_\mathrm{emb}$, respectively. 
    Here, we show the results of $1M_\oplus$ embryos around $0.4 \au$.
    %obtained with $a_\mathrm{p}=10 \au$ and $M_\mathrm{emb}=1M_\oplus$.
    }
    \label{fig: time_orbit_Embryos}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
  \begin{center}
    \includegraphics[width=80mm]{fig/Multi/Embryos_psMemb.png}
    \caption{
    Same as Fig.~\ref{fig:fitting} but with the blue plots showing the results for embryos instead of the planetesimal disk. 
    We use 5 embryos for each simulation and sum up the collision fraction. 
    The upper panel shows the case with 1 $M_{\oplus}$ embryos, and the lower panel shows the case with 0.1 $M_{\oplus}$ embryos.
    For comparison, we also plot the results for the planetesimal disk. 
    The initial inclination of the planetesimal disk is equal to the reduced hill radius of embryos. 
    }
    \label{fig: embryos}
  \end{center}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the simulations discussed above, we treated planetesimals as test particles. 
To investigate the effects of mutual gravitational interactions, we perform additional simulations using five equal-sized embryos instead of the planetesimal disk.
We set the mass of each embryo $M_\mathrm{emb}$ to $1 M_\oplus$ and $0.1 M_\oplus$.
The embryos' mean density is set to $5.5 \mathrm{g/cm^3}$, and the initial semi-major axis of the innermost embryo is an input parameter $a_\mathrm{emb,0}$.
The rest of the embryos are distributed with the radial orbital separation of 10 mutual Hill radii.
The eccentricity and inclination are given by the Rayleigh distribution with $\left \langle e_0^2 \right \rangle^{1/2} = 2 \left \langle \sin^2 i_0 \right \rangle^{1/2} = 10^{-3}$, and the orbital angles are set randomly.
We perform simulations with 40 different seeds for each $a_\mathrm{emb,0}$ and assume perfect mergers for collisions.

Due to the mutual gravitational interactions, the eccentricity and inclination are excited to $\sim h_\mathrm{emb}$, which is a reduced mutual Hill radius $h_\mathrm{emb}= (2 M_\mathrm{emb}/3 M_\mathrm{s})^{1/3}$.
When the embryos' inclination reaches $\left \langle \sin i \right \rangle \sim h_\mathrm{emb}$ it evolves similarly to the planetesimals.
Figure~\ref{fig: time_orbit_Embryos} shows the time evolution of the geometrical mean of eccentricities and inclinations of embryos.
The embryos' inclination increases with time more rapidly than that of planetesimals in the early evolution stage $t\lesssim10P_\mathrm{orb,p}$ because the mutual interactions between the embryos dominate the inclination evolution.
After that stage, the inclination evolution follows that expected from eq.~(\ref{eq:TimeEvolution_Inc}) with $\left \langle \sin i_0 \right \rangle \sim h_\mathrm{emb}$.

Figure~\ref{fig: embryos} shows the collision fraction $F_\mathrm{col,emb}$ as a function of semi-majot axis. $F_\mathrm{col,emb}=M_\mathrm{col, tot}/M_\mathrm{emb, tot}$ where $M_\mathrm{col, tot}$ is the total mass of the embryos accreted by the eccentric planet. $M_\mathrm{emb,tot}=200 M_\mathrm{emb}$ is the total mass of embryos used for each $a_\mathrm{emb,0}$.
We also plot the accretion fraction $F_\mathrm{acc}$ obtained in the simulations using the planetesimal disk with $\left \langle \sin^2 i_0 \right \rangle^{1/2} = h_\mathrm{emb}$.
We find that the collision fraction $F_\mathrm{col,emb}$ is comparable to the accretion fraction $F_\mathrm{acc}$.
Therefore, we can conclude that the collision probability of embryos is also given by $P_\mathrm{col}^\prime$ with $\left \langle \sin i_0 \right \rangle=h_\mathrm{emb}$.







